What makes Ethereum blockchain transactions be processed fast or slow? An empirical study

The Ethereum platform allows developers to implement and deploy applications called Dapps onto the blockchain for public use through the use of smart contracts. To execute code within a smart contract, a paid transaction must be issued towards one of the functions that are exposed in the interface of a contract. However, such a transaction is only processed once one of the miners in the peer-to-peer network selects it, adds it to a block, and appends that block to the blockchain This creates a delay between transaction submission and code execution. It is crucial for Dapp developers to be able to precisely estimate when transactions will be processed, since this allows them to define and provide a certain Quality of Service (QoS) level (e.g., 95% of the transactions processed within 1 minute). However, the impact that different factors have on these times have not yet been studied. Processing time estimation services are used by Dapp developers to achieve predefined QoS. Yet, these services offer minimal insights into what factors impact processing times. Considering the vast amount of data that surrounds the Ethereum blockchain, changes in processing times are hard for Dapp developers to predict, making it difficult to maintain said QoS. In our study, we build random forest models to understand the factors that are associated with transaction processing times. We engineer several features that capture blockchain internal factors, as well as gas pricing behaviors of transaction issuers. By interpreting our models, we conclude that features surrounding gas pricing behaviors are very strongly associated with transaction processing times. Based on our empirical results, we provide Dapp developers with concrete insights that can help them provide and maintain high levels of QoS.

==> bios.tex <==
\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/mike.png}}]{Michael Pacheco} \goliva{Update your bio if needed (same for other co-authors).} is a MSc student at the School of Computing of Queen's University in Canada under the supervision of Dr. Ahmed Hassan and Dr. Gustavo A. Oliva. His research at the Software Analysis and Intelligence Lab (SAIL) focuses on understanding and evaluating the transaction processing mechanism of Ethereum.
\end{IEEEbiography}
		
\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/gus.png}}]
	{Gustavo A. Oliva} is an Adjunct Professor at the School of Computing of Queen's University in Canada. Gustavo leads the blockchain research team at the Software Analysis and Intelligence Lab (SAIL). In addition to blockchain, he also conducts empirical studies in the fields of software ecosystems (e.g., npm), software evolution, and explanaible AI. Gustavo received his MSc and PhD degrees from the University of São Paulo (USP) in Brazil under the supervision of professor Dr. Marco Aur{é}lio Gerosa. More information at: \url{https://www.gaoliva.com}
\end{IEEEbiography}

\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/gopi.jpg}}] {Gopi Krishnan Rajbahadur} is a Senior Researcher at the Centre for Software Excellence at Huawei, Canada. He holds a PhD in computer science from Queen's University, Canada. He received his BE in computer Science and Engineering from SKR Engineering college, Anna University, India. His research interests include AI Engineering, Software Engineering for Artificial Intelligence (SE4AI), Artificial Intelligence for Software Engineering (AI4SE), Mining Software Repositories (MSR) and Explainable AI (XAI).
\end{IEEEbiography}
	
\vspace{-7ex}

\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bios/ahmed.png}}] {Ahmed E. Hassan} is an IEEE Fellow, an ACM SIGSOFT Influential	Educator, an NSERC Steacie Fellow, the Canada Research Chair (CRC) in Software Analytics, and the NSERC/BlackBerry Software Engineering Chair at the School of Computing at Queen’s University, Canada. His research interests include mining software repositories, empirical software engineering, load testing, and log mining. He received a PhD in Computer Science from the University of Waterloo. He spearheaded the creation of the Mining Software Repositories (MSR) conference and its research community. He also serves/d on the editorial boards of IEEE Transactions on Software Engineering, Springer Journal of Empirical Software Engineering, and PeerJ Computer Science. More information at: \url{http://sail.cs.queensu.ca}.
\end{IEEEbiography}

==> discussion_old.tex <==
\section{Discussion}
\label{sec:discussion}

In the following section, we discuss the implication drawn from our findings in the previous sections. 

% \mike{need to figure out how to remove the log of these plots. they seem to be based on matplotlib python package, so i can begin from there..}

% we're going to use this in the discussion to highlight that the design of our model + the use of bleeding edge interpretation techniques (SHAP)
% yield an interpretable model that developers can use in practice to understand each prediction given by the model. 
% then you can show two txs. one where the shaps are aligned with the global view of feature importances and another  tx that significantly deviates from the global feature importance (e.g., some tx for which the top SHAPs are features with ranks 5+ or something).
\gopi{I disagree with implication 1. And the general idea that we are building explainable/or a simple white box model for people to use. In my opinion, this study should simply focus on saying that we want to observe which features affect the transaction processing times and how it does so, so that DApp developers could leverage those findings. If we say they can use our models, except for features we don't really provide anything. We just say build a RF and use SHAP. That is in my opinion not an implication of our finding. Also, when dichotomy between the global and local interpretation exist what should the Dapp developer follow? I think we don't need to go down this route and these Fig-10 and Fig-11 don't really add anything to the narrative. I also recommend to clean up everywhere about we present a model for the DApp developers to use. We provide findings that they can leverage and insights on trends..So I recommend dropping implication 1 } 
\mike{I see your point and mostly agree, as we dont propose a new model or anything like that. As you said I think this implication should instead focus on noting the proposal for such a framework/guidelines, as it makes sense that if anything we are contributing a framework for others to follow (sound model construction approach followed by canonical interpretation methods) that can be used to understand trends to yield similar insights to ours including the findings that we report. But then if we are mentioning that the framework can be used to produce these or similar findings, maybe it should just be in the conclusion. Again, the current version of the implication sounds a bit odd as we mention models twice, so doesnt make as much sense to me. I also agree that the global and local interpretations (i.e. global SHAP vs waterfall) are kind of confusing as to which ones DApp devs should follow. I believe our initial plan plan was to manually investigate some of the waterfall plot results to find 1 example that mostly agrees with the global view, and one that does not. I then wrote an RQ that said the important features change depending on the context of the network, but even that approach holds the same confusion and Im unsure its worth selling it that way. So yes we might need to think about this a bit more.}\goliva{I see. I agree with a lot of the things you've said. I don't agree with the dichotomy argument though. A global importance is always an approximation - i.e., it doesn't mean that top features will be important for every single transaction (it will for sure be the case for *most* transactions though - by construction). So I don't see a problem there. There is a need for models to be accountable if such models are to be used in practice. I don't see anything wrong in saying that our overall approach (model construction + interpretation method) fulfills that gap. However, as I do see your point. Selling it as an implication is likely 'too much'. And maybe even open doors for `reviewer 2 species' (such as Gopi :-p) to argue. My whole point was that not that many people are actually familiar with SHAP and know that you can have 'accountability' for every tx prediction via waterfall plots. So what I'd suggest is something in between. More specifically: (1): remove this implication, (2) as Gopi beautifully suggested, under Observation 4, add a sentence right before the last one saying something like 'As an illustrative example, Figure 11 depicts a transaction whose primary predictors are low-ranked features.". I'd keep the 'contributions to practice' (in the introduction) as is in the introduction. But let's see what Ahmed says, maybe we just tone it down a bit."}


\implication{Our approach results in models that \dapp developers can use in practice to understand each prediction given by our models.} \mike{Not 100\% sure what to do here about this implication, since it sounds like Ahmed doesnt like this implication either. Thoguhts? Also our old discussion here is commented out above this text}
To follow the goal of our study, we carefully design and follow an interpretable model construction approach and also use SHAP, a relevant interpretation technique, to yield interpretable predictions. Our approach thus yields models that \dapp developers can use in practice to understand how the resulting predictions are made, which can help them set gas prices for their transactions. In Figures~\ref{fig:waterfall-similar} and~\ref{fig:waterfall-deviate}, we use a waterfall plot to quantify the amount of impact that each feature holds on the resulting prediction of our model for two specific transactions, as a method of demonstrating the practicality of our results. 
%\mike{for this "deviate" instance, we didnt discuss a specific way to select it. im not sure if we can use SK to rank SHAP values for a single instance (as opposed to samples), and then compare the ranks to the global view using kendall tau. i feel there is a better way we can do this}

Figure~\ref{fig:waterfall-similar} focuses on a transaction \goliva{Add txn hash in the footnote. I think you sent me this info in Hangouts at some point} \mike{I am leaving this untouched since we should first discuss Gopi's concern above, and we may change the tx according to Gustavo's suggestion below (to find a tx with top3 match)}with SHAP values that closely resemble the global feature importances of our model (Figure~\ref{fig:feature_importance}). In this case, we can see how concrete values for each of the features impact the prediction. For example, in this case we see that the value of 0 for \textit{med\_num\_below\_120\_perc} increases the prediction value, while conversely the moderate value of \textit{std\_num\_below\_120} decreases the prediction. \goliva{Ideally, you should pick a txn where the top-3 match to make our point crystal clear (here only top-2 match.)}\mike{I am leaving this untouched since we should first discuss Gopi's concern above)}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{images/discussion/wfall1-nolog.pdf}
    \caption{A waterfall plot for a transaction with SHAP values that closely reflects the global feature importances.}    
    \label{fig:waterfall-similar}
\end{figure}

Figure~\ref{fig:waterfall-deviate} depicts a transaction with SHAP ranks that do not conform to the global feature importances from Figure~\ref{fig:feature_importance}. Specifically for this transaction, our model finds the value of the \texttt{std\_pending\_pool\_120} (global rank 12) to hold the highest explanatory power of transaction processing time. The high value for this feature results in a reduction in the prediction value. However, such a feature only moves the prediction back by 0.06 minutes = 3.6 seconds. In fact, the other 21 omitted features contribute (together) with a higher SHAP value compared to \texttt{std\_pending\_pool\_120}. This is thus a case where the resulting prediction is driven by the small contribution of each and every feature.

These two waterfall plots illustrate how importances vary between instances, and how they are dependent on the values that each of the features hold (which change based on the state of the Ethereum blockchain). Using our approach, \dapp developers can continue to leverage this information to understand why models produce a particular prediction (accountability), and thus plan the execution of the transactions in their applications.

\begin{figure}[!htbp]
\centering
    \includegraphics[width=\linewidth]{images/discussion/wfall2-nolog.pdf}
    \caption{A waterfall plot for a transaction with SHAP values that deviates from the global feature importances. The top feature \texttt{std\_pending\_pool\_120} has a global rank of 12 (see Figure~\ref{fig:feature_importance}). \goliva{Add a footnote with the hash of this transaction}}
    \label{fig:waterfall-deviate}
\end{figure}

\implication{\dapp developers should primarily consider recent historical information regarding gas prices of transactions in the recent past to achieve fast processing times.} In Section~\ref{sec:rq} we observe that features within the historical dimension are heavily relied upon by our model for its resulting predictions. In particular, the \textit{med\_num\_below\_120\_perc}, \textit{std\_num\_below\_120}, and \textit{num\_same\_1\_perc} features are ranked as the top 3 most important features, all of which are historical metrics that relate to gas price (a behavioural feature) from transactions found within the previous 120/1 block(s). Such historical information is far more important than the gas price per se, which is ranked only 9th in terms of global importance (Figure~\ref{fig:feature_importance}). For instance, \dapp developers can measure the \textit{med\_num\_below\_120\_perc} feature themselves to ensure that they execute transactions with gas prices greater than or equal to the value of that transaction, to reduce processing times. We note here that 120 blocks typically correspond to 30 minutes, as one block is appended to the Ethereum blockchain every 15 seconds on average. 

On the other hand, our model consistently shows that features in the contextual dimensions generally do not help the resulting prediction. We note here that although this is true, the features engineered in the historical dimension which use information from the previous 120 blocks can act as a definition for the state of the Ethereum blockchain at a specific point in time. For example, the \textit{gas\_price\_gwei} and \textit{med\_num\_below\_120\_perc} combined reflect how many transactions in the previous 120 blocks were processed with gas prices lower than the transaction in question, which can be interpreted as a simple measurement of network traffic.

%Following, \dapp developers can choose to ignore this information, and put more effort in monitoring historical gas price information instead.
% \mike{give examples of values for these and how they can reflect the network util/congestion., eg when both values are low, high, then highlow/lowhigh - what can these all mean?}
%    For this, the top 3 metrics do act as a "contextual" feature as well, since the "median and std of the percentage of prev txs with gas prices under the current one" features do act as "network utilization" information. this is importnat to note in combination that pending pool + network utilization do not have much explanatory power alone.
% \implication{Contextual information (time of day, difficulty of the network at a point in time, pending pool, network utilization) do not explain processing time as well as historical or behavioural features.}

% \implication{\dapp developers may need to focus on their experience in the Ethereum blockchain (i.e., nonce value), along with the allocation of gas price.} 
\implication{\dapp developers should also avoid designing applications which implement and or invoke smart contract functions which consume large amounts of gas.} 
%It is natural that \dapp developers can achieve fast processing times by assigning high gas prices to their transactions. This is because every transaction needs to be paid for through a transaction fee, calculated by \textit{gas usage} $\times$ \textit{gas price}, and miners are rewarded a portion of this amount for processing the transaction. This calculation also suggests that fast processing times can be achieved by invoking smart contract functions that use high amounts of gas. However, Figure \ref{fig:feature_importance} displays that our model considers features related to historical gas price features (including \textit{gas\_price\_gwei} itself) to hold the highest importance. On the other hand, the figure displays that the \textit{tx\_gas\_limit} (transaction gas limit) and \textit{std\_func\_gas\_usage\_120} (standard deviation of historical gas usage of the smart contract function in the previous 120 blocks) features are deemed much less important (ranked 21 and 25 respectively). 
This suggests that transactions with high gas prices are prioritized by miners over the amount of gas they will potentially consume. If a \dapp developer designs an application which invokes multiple smart contract functions that each consume large amounts of gas, their transactions will still require high gas prices to be processed timely. Such \dapps might be costly and potentially unfeasible to maintain. Therefore, \dapp developers should focus on utilizing smart contract functions consuming minimal amounts of gas, and using them with transactions holding competitive gas prices. However, heavy computations may be required in smart contracts for specific \dapp use cases. In these scenarios, \dapp developers should focus on balancing invocations of such functions by dividing their computation into multiple functions. These divided functions can then be invoked individually with transactions that are each assigned high, competitive gas prices to ensure fast processing times.


% \hl{As miners receive a reward for processing transactions based on the transaction fee, calculated by \textit{gas usage} $\times$ \textit{gas price}, it is commonly expected miners prioritize transactions with higher gas prices than others. However, the transaction fee is also calculated from the \textit{gas usage}, which relates to the \textit{gas limit} set on a transaction. If the \textit{gas limit} of a transaction is set lower than the required amount of gas units needed to execute code in a smart contract, the transaction can fail resulting in an \textit{out of gas failure}. In this case, miners risk processing a transaction that will fail, and as a result will not yield as much reward as processing successful transactions. Even so, our model does not consider the \textit{tx\_gas\_limit} feature to hold strong explanatory power for predicting transaction processing time.

% Interestingly, our model considers the \textit{tx\_nonce} (defined as the number of transactions executed by the sender of a transaction) to be of considerable importance compared to the \textit{tx\_gas\_limit}. This suggests that miners may prioritize processing transactions from experienced users, as they believe there is lower probability of these transactions resulting in an \textit{out of gas failure}, or other failures in general. This is also a more convenient approach, since miners would need to store massive amounts of historical information regarding the gas usage consumed by several different smart contract functions on the fly. In turn, monitoring and prioritizing the \textit{tx\_nonce} of transactions might provide miners with a more practical alternative.} 
%\goliva{Rewrite this one. So the discussion always needs to be from the tx issuer point of view. The key point here is that tx fee is a function of both gas usage and gas price. Yet, the model is showing that historical gas price features (and even the gas price per se) are far more important than gas usage (proxified by std\_func\_gas\_usage\_120, which is correlated with med\_func\_gas\_usage\_120). This means miners don't care about (or don't look at gas usage). Yet, again, the tx fee takes gas usage into account. So as a developer, this becomes tricky. If you have a function that burns a lot of gas, you're screwed up, because only to speed up the tx is to increasing gas price, which will make your tx super expensive. So devs should avoid having ``heavy txs'' (txs that burn a lot of gas). this means contracts should be designed such that a tx never burns too much gas (otherwise he can't increase gas price without suffering too much). I'm being verbose here, but you get the point.This is a very important aspect actually! Look at the discussion in Zarir's gas usage paper, as we actually reach the exact same conclusion there.\gopi{Gustavo's point is really nice. Once you add it, I can take a look at it}\mike{great perspective, thank you. New text is above this comment. Ive kept the old paragraph in the text just in case}}

% We can say here that miners may be prioritizing gas price only, as gas limit offers little explanatory power. This is important since a miner can choose a tx that is prone to an out of gas failure. However, it seems maybe they prioritize tx nonce, or the experience of the sender, which would mean they expect that experienced senders avoid these failures. A PEP for tx nonce and processing time would also be cool to see how they relate (probably positive relationship, maybe until a certain nonce value).  






 


==> extra.tex <==
Moreover, very limited information is provided regarding the design and validation of these models, making it unclear what factors influence processing time the most. Finally, designing a new model that outperforms the predictions produced by these state-of-the-practice tools has the potential to drastically improve the economics behind \dapps. 

-----------------

Finally we investigate how network utilization influences transaction processing times. We quantify network utilization using the following metric:

\begin{scriptsize}
\begin{equation}
    \begin{aligned}
      NetworkUtilization(B_i, t) = \dfrac{\sum_{i-t}^{i-1}BlockFilledPercentage(B_i)}{t} \\
      BlockFilledPercentage(B) = \dfrac{gasUsed(B)}{gasLimit(B)} * 100
    \end{aligned}
\end{equation}
\end{scriptsize}

As shown above, the network utilization metric is a function of the $BlockFilledPercentage(B)$ metric. $BlockFilledPercentage(B)$ is defined as the ratio between the \textit{block gas used} over the \textit{block gas limit} of a given block $B$. The network utilization is then defined as taking the average of $BlockFilledPercentage$ over the \textit{t} blocks that were appended before block $B_i$, where \textit{i} denotes the \textit{block number}. We use $t = 120$ for this project, which in units of time represents approximately 30 minutes (as it is assumed that the Ethereum blockchain appends a new block to the chain every 15 seconds).

\smallskip \observation{Cheaper transactions are more susceptible to delays in processing time when the network utilization increases.} Figure \ref{fig:net_cong} depicts a heatmap in which we compare the median processing time per block (i.e., the median of the processing times of all transactions in a given block) with the network utilization. A visual inspection of the heatmap indicates that most of the observations lie in the upper left corner of the figure (note the red hexagons), with no apparent correlation between the two variables. Indeed, the Spearman's rho indicates that there is only very weak (0.05) correlation between them.

\begin{figure}[!htbp]
\centering
  \includegraphics[width=\linewidth]{rq1/net_cong_vs_median_pr_time.pdf}
  \caption{Heatmap contrasting the median transaction processing time per block with the network utilization level.}
  \label{fig:net_cong}
\end{figure}

We conjecture that network utilization impacts only transactions with cheaper prices. Therefore, we investigated how processing times vary for different price categories and different network utilization levels. The results are depicted in Figure \ref{fig:net_cong_range_vs_med_pr_time}. The figure corroborates our conjecture. As network utilization increases, the processing time of cheaper transactions tend to increase (e.g., note the red boxplots and their medians). Expensive and very expensive transactions are remarkably less impacted by network utilization. Interestingly, for all gas price categories, the median processing time of transactions is lower for an utilization level of (90, 100] compared to the (80, 90] utilization level. We hypothesize that miner nodes start working more intensively when the network is being very highly utilized (e.g., when it shows first signs of congestion).

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{rq1/net_cong_vs_price_category.pdf}
    \caption{Relation between network utilization on gas prices}
    \label{fig:net_cong_range_vs_med_pr_time}
\end{figure}



==> old/04c-model-construction.tex <==
%\subsection{(Step-3) Model Construction}

%After obtaining the new feature set resulting from our preprocessing pipeline in Section \ref{subsec:feature-preprocessing}, we transition toward building our prediction model using this feature set. The main steps of constructing our models include first choosing to build a linear regressor with restricted cubic splines, the process of estimating the budget for degrees of freedom, and finally the process of allocating knots within this budget. In this section we describe each of these steps in more detail below.

%\smallskip \noindent \textbf{3a. Model choice} \goliva{explain what a linear regression with restricted cubic splines is and why we chose it}\mike{added below}
%We choose to build a linear regression model with restricted cubic splines. Linear regression models are inherently transparent in their design and easily interpretable \cite{molnar2019}. We also use restricted cubic splines to allocate the budgeted degrees of freedom to each of the features. Restricted cubic splines... \mike{paging Gopi for this explanation here :) also here is the citation for the book} \citet{Harrell2015}. The ols function from the rms package is used to create the linear regression models.

%\smallskip \noindent \textbf{3b. Budget estimation for degrees of freedom (knots)} We estimate our budget for degrees of freedom by calculating $n/15$ following the work of \citet{Harrell1985}, where n is the number of rows in the dataset in each window. Every window contains a unique amount of transactions, which results in a different value in the budget for each window. By allocating an amount of knots to our features that remains below the budget, linear regression model built will avoid overfitting the data it is trained on. \mike{will read more about this}

%\smallskip \noindent \textbf{3c. Allocate degrees of freedom (knots)} Finally, we look to allocate degrees of freedom to independent features by allocating knots to them. To do this, we leverage the spearman2 function of the rms package. This function calculates the Spearman multiple $p^2$ between each independent variable and the dependent variable. If the Spearman multiple $p^2$ value is large, there is a strong non-monotonic or nonlinear relationship between that independent variable and dependent variable pair. The independent variables in these pairs  would benefit the most from being assigned knots. We first calculate the total degrees of freedom, or budget, so we can allocate knots to our feature set while maintaining a sum of knots less than this budget. We choose to allocate knots using the rcs function from the rms package. We decide the number of knots to allocate to each independent feature based on the value of their Spearman multiple $p^2$ score, followed by an analysis on the relationship between the independent feature and the dependent feature. We repeat this process across all windows, and take the average multiple $p^2$ score across all windows, which reveals strong relationships (in order of $p^2$ descending) between transaction processing time and\textit{closest\_txn\_pr\_time}, \textit{gas\_price\_gwei},  and \textit{gas\_price\_category\_very\_cheap} respectively. We ignore \textit{gas\_price\_category\_very\_cheap}, which can only have two unique value as it is a one-hot encoded version of the gas price category, and can only be one of two values (0/1, indicating true/false). We list the spearman $p^2$ values in Table \ref{tab:knots_spearman_p} in Section \ref{appendix:knot-allocation} of the Appendix. 

==> old/extra.tex <==
Moreover, very limited information is provided regarding the design and validation of these models, making it unclear what factors influence processing time the most. Finally, designing a new model that outperforms the predictions produced by these state-of-the-practice tools has the potential to drastically improve the economics behind \dapps. 

\smallskip \observation{Cheaper transactions are more susceptible to delays in processing time when the network utilization increases.} Figure \ref{fig:net_cong} depicts a heatmap in which we compare the median processing time per block (i.e., the median of the processing times of all transactions in a given block) with the network utilization. A visual inspection of the heatmap indicates that most of the observations lie in the upper left corner of the figure (note the red hexagons), with no apparent correlation between the two variables. Indeed, the Spearman's rho indicates that there is only very weak (0.05) correlation between them.

\begin{figure}[!htbp]
\centering
  \includegraphics[width=\linewidth]{rq1/net_cong_vs_median_pr_time.pdf}
  \caption{Heatmap contrasting the median transaction processing time per block with the network utilization level.}
  \label{fig:net_cong}
\end{figure}

We conjecture that network utilization impacts only transactions with cheaper prices. Therefore, we investigated how processing times vary for different price categories and different network utilization levels. The results are depicted in Figure \ref{fig:net_cong_range_vs_med_pr_time}. The figure corroborates our conjecture. As network utilization increases, the processing time of cheaper transactions tend to increase (e.g., note the red boxplots and their medians). Expensive and very expensive transactions are remarkably less impacted by network utilization. Interestingly, for all gas price categories, the median processing time of transactions is lower for an utilization level of (90, 100] compared to the (80, 90] utilization level. We hypothesize that miner nodes start working more intensively when the network is being very highly utilized (e.g., when it shows first signs of congestion).

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{rq1/net_cong_vs_price_category.pdf}
    \caption{Relation between network utilization on gas prices}
    \label{fig:net_cong_range_vs_med_pr_time}
\end{figure}



==> old/interpretation.tex <==
\section{RQ3: Design and validation of our proposed model}
\label{appendix:rq3}

\smallskip \noindent \textbf{a) Feature engineering.}  We engineered 18 features along 4  dimensions. In Table \ref{tab:features}, we present the features and the rationale behind them.

\begin{table*}[!htbp]
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Features used to build our models along with their rationale.}
\label{tab:features}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llp{4cm}p{\linewidth/2}} \hline
\textbf{Type} & \textbf{Name} & \textbf{Description} & \textbf{Rationale} \\ \hline
Temporal & \texttt{day} & Day of the week (one hot encoded) & Time of the transaction may reveal network congestion \\
 & \texttt{hour} & Hour of the day (label encoded) &  \\ \hline
Contextual & \texttt{to\_contract} & If the transaction is toward contract or not & Contract transactions may be prioritized differently by miners, or have longer execution times \\
 & \texttt{contract\_bytecote\_length} & Size of contract in bytes & Larger size may result in an increase in execution time, and thus processing time \\
 & \texttt{is\_erc20} & Whether the contract being targeted is ERC20 contract & Different contracts (erc20/erc721 = token) may have different properties W.R.T processing + prioritization \\
 & \texttt{is\_erc721} & Whether the contract being targeted is ERC721 contract &  \\
 & \texttt{contract\_block\_number} & The block number that the contract being targeted was created in & Older contracts may execute inefficient code, which may impact times \\
 & \texttt{net\_util} & Network utilization & Network utilization affects processing times of txs. with lower gas prices (RQ1) \\ \hline
Behavioural & \texttt{nonce} & Transaction counter of the user & User experience may be associated with setting inappropriate gas price, or nonce may be prioritized differently by miners \\
 & \texttt{gas\_price\_gwei} & Gas price set by the user in GWEI & Directly related to transaction processing times \\
 & \texttt{gas\_limit} & Gas limit set by the user & Miners may avoid transactions if they think it might result in out of gas error \\
 & \texttt{input\_length} & Size of input data in bytes & Longer inputs may take longer to execute and process \\
 & \texttt{function} & Function to be invoked from contract & Different functions execute different code, which may impact these times \\ \hline
Historical & past\_avg & Past average processing time of 100 of the transactions with the most similar gas prices within the previous 120 blocks & Past average, standard deviation and median of processing times of the most similar transactions within the previous 120 blocks will give the model a sense of how long the current transaction should be taking to be processed. Should also capture any impacts on processing time the network may be facing. \\
 & \texttt{past\_std\_dev} & Past standard deviation processing time  of 100 of the transactions with the most similar gas prices within the previous 120 blocks &  \\
 & \texttt{past\_med} & Past median processing time  of 100 of the transactions with the most similar gas prices within the previous 120 blocks &  \\
 & \texttt{num\_same\_price} & Number of transactions at the same gas price as the transaction found within the previous 120 blocks & Discrepancy between common or uncommon gas prices should help differentiate between processing times of such transactions \\
 & \texttt{num\_above} & Number of transactions above the gas price of the transaction found within the previous & \\ \hline
\end{tabular}
}
\end{table*}

\smallskip \noindent \textbf{b) Model choice.} We devise a regression model that aims to predict transaction processing time. Following the recommendation from \citet{Tantithamthavorn18}, we try different learners: Linear Regression, Random Forests, and LightGBM. Linear Regression is the simplest of the three and inherently interpretable. Random Forest is an ensemble method based on decision trees that has been extensively used with success in Software Engineering research \citep{Yu19, Calefato19, Bao19}. LightGBM is a cutting-edge Gradient Boosted Decision Trees algorithm developed by Microsoft \citep{LightGBM} and that has been used by several winners of machine learning competitions on Kaggle. For Linear Regression and Random Forests we used the implementations from the \texttt{scikit-learn} Python package\footnote{\url{https://scikit-learn.org}}. For LightGBM, we used Microsoft's official Python implementation\footnote{\url{https://github.com/microsoft/LightGBM}}.

\smallskip \noindent \textbf{c) Metrics for accuracy and feature importance.} To measure the accuracy of our model, we choose the same metrics that we employed in RQ2 (Section \ref{subsec:rq2}). That is, we measure accuracy in terms of the Absolute Percentage Error (APE). In addition, for information purposes, we also report the Mean Absolute Percentage Error (MAPE) and the Mean Absolute Error (MAE) of our model. We also report the goodness-of-fit of our model by means of the $R^2$ score. 

As for feature importance, we calculate \textit{permutation importance}. Permutation importance is a model-agnostic feature importance method. First, the performance of a model is calculated on the original training dataset \goliva{which metric is being used here? in R, randomForests use MSE}. Next, a feature (column) in the training dataset is randomly permuted and the performance of the model is recalculated. The delta between the two performances indicate the importance of the feature. This process is repeated for each feature in the dataset, such that importance is determined for the entire feature set. The rationale is that, if a feature contributes significantly to the output of the model, perturbating such a feature (while still preserving its distribution) should significantly impact the performance of the model. 


To validate the results of our model, we first compute the MAPE, MAE, and $R^2$ score across all test sets. We then also compare the predictions made by our models to that of the competitor predictions. We do this by first obtaining four subsets of transactions that both our models and a competitor model predicted processing times for - one subset for each competitor prediction, which contains predictions for each bootstrap. We then compute the three metrics for our models and each competitor model and compare them. Lastly we compute the absolute errors for our models and each of the competitor models, generate two columns of the AEs of the constructed models and that of the competitor predictors, and run Scott Knott ESD on these AEs to determine if the AEs contain a statistically significant difference in effect size. \mike{added this paragraph to define our comparison process} 

\smallskip \noindent \textbf{c) Model validation and hyper-parameter tuning.} To account for the historical nature of some of our features, we employ a sliding-time-window-based model validation technique \citep{Lin18}. More specifically, we use a window of three days, where the two first days are used for training and the third day is used for testing. We then slide the window one day and repeat until the complete period is evaluated (i.e., November 21st 2019 until December 09th, 2019). A schematic is shown in Figure \ref{fig:sliding-window}.

\begin{figure}[!htbp]
  \centering
    \includegraphics[width=1.0\linewidth,keepaspectratio=true]{images/appendix/sliding-window.pdf}
    \caption{Our sliding-time-window-based model validation.}
    \label{fig:sliding-window}
\end{figure}

We then proceed to the training process, which implements a sliding window technique \citep{Lin18} for testing and training sets. This technique builds several models by chunking the data by timestamp into groups which fall within a specific time period or window. A model is then built using this train test split, and finally the window is moved forward in time. This processes repeats until the latest date of the transaction within the dataset is reached. This process first consists of an analysis of the effect of various ranges of the sliding window technique on the performance of the various models. The sliding window ranges that result in the best average performance of the models is chosen. For each time window, a bootstrap is performed on the training data for 100 \mike{updated all metrics with 100 bootstrap iterations} iterations, using the same constant set for testing data. The following performance metrics from the models resulting from the bootstrap and time window iterations include: $R^2$ score, mean absolute error, and mean absolute percentage error. The feature importances for the random forest and gradient boosted decision tree models are also saved after each bootstrap, which at the end is used to compute the most important features according to the respective models by using Scott Knott ESD on the importances.

The experiments of comparing sliding windows and the train and test bounds used to train the models reveal that the models perform the greatest when they are trained using: i) two days of training, ii) the following day for testing, and iii) sliding the time window by one day for each iteration. We expect this outcome may be due to the fact that two days gives the models enough data to generalize to the relationships of transaction processing times, but not enough data for them to overfit to the processing times occurring within the window.

\smallskip \noindent \textbf{d) Feature preprocessing and filtering.} For preprocessing, we first apply a log normalization to both the independent and dependent features in our dataset. Correlation and redundancy analyses are then performed on the features we have collected and chosen to include within our models. Both analyses are performed using the RMS package in R, where a threshold of 0.8 is used for the correlation analysis to indicate very strong correlation. 

The results of analyzing redundant variables amongst the selected feature set indicate that the outcomes of i) \textit{to\_contract}, and ii) \textit{past\_med} features can be predicted from the other features in the set. The \textit{to\_contract} feature is redundant as other features will remain constant. An example of this is the \textit{contract\_bytecode\_length} feature, where if \textit{to\_contract} = 0, \textit{contract\_bytecode\_length} = 0 as well. As for \textit{past\_med}, this feature is most likely explained through the features \textit{past\_avg} and \textit{past\_std\_dev}. The results of redundancy analysis can be found in Table \ref{tab:redundancy_analysis}. \mike{updated this text}

\begin{table}[!htbp]
\centering
\caption{Results of redundancy analysis on the selected feature set used to train the predictive models.}
\label{tab:redundancy_analysis}
\begin{tabular}{ll}
\hline
\multicolumn{1}{c}{\textbf{Iteration}} & \multicolumn{1}{c}{\textbf{Redundant Variable}}\\ \hline
1 & to\_contract \\ 
2 & past\_med\\ \hline
\end{tabular}
\end{table}

Correlation analysis performed on the set of features used to build the predictive models reveal that the feature \textit{past\_std\_dev} and \textit{past\_avg} are strongly correlated, with a score of 0.96. Similar to the results of the redundancy analysis, \textit{past\_std\_dev} and \textit{past\_avg} are directly related and actually strongly correlated, most likely since the standard deviation is a metric that is calculated using the average as reference. We choose to remove \textit{past\_std\_dev}, as \textit{past\_avg} should allow the models to make more accurate predictions of transaction processing time as opposed to \textit{past\_std\_dev}. The results of correlation analysis can be found in Table \ref{tab:correlation_analysis}. \mike{I updated this, however not sure what rationale we should write to explain why we removed std dev and not past avg}

\begin{table}[!htbp]
\centering
\caption{Correlated variables over the 0.8 threshold.}
\label{tab:correlation_analysis}
\begin{tabular}{lll}
\hline
Feature 1      & Feature 2 & Correlation Score \\ \hline
past\_std\_dev & past\_avg & 0.96             \\\hline
\end{tabular}
\end{table}



==> prelim-study.tex <==
\section{Preliminary Study: \PrelimStudy}
\label{sec:prelim-study}

\noindent \textbf{Motivation.} Before interpreting our random forest models, we first need to determine whether our engineered features provide our model with enough explanatory power.

\smallskip \noindent \textbf{Approach.} To determine the explanatory power of our model, we calculate its $R^2$. The $R^2$ determines how much of the total variability in processing times is explained by our model, serving as good proxy for explanatory power.

To compute the adjusted $R^2$ of our constructed random forest model, we apply the model construction steps outlined in Section~\ref{sec:model-construction} then setup a model validation pipeline that splits data into train, test, and validation sets (Figure~\ref{fig:model-validation}). Our train dataset needs to be as large as possible, otherwise our model cannot identify possible seasonalities in the data (e.g., evaluate the influence of the \textit{day of the week} in transaction processing times) nor changes in the blockchain context (e.g., network conditions are unlikely to change in small periods of time). We thus define the training set as the first 28 days of data, the validation set as the 29\textsuperscript{th} day, and the test set as the final day. We split the data along its temporal nature to avoid data leakage \gopi{cite Yingzhe's paper on AIOps}\mike{Done}\cite{Yingzhe2021}. We then use the training set to generate 100 bootstrap samples (i.e., samples with replacement and of the same length as the training set). For each bootstrap sample, we first fit a random forest \gopi{decide if we are using random forest or RandomForest and be consistent everywhere}\mike{Done, chose model}model on that sample. Next, we use the validation set to hyperparameter tune that model as recommended by prior studies to ensure that our constructed model fits the data optimally. For hyperparameter tuning we choose the \texttt{RandomizedSearchCV} \cite{Bergstra2012} from \texttt{scikit-learn}\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.model_selection.RandomizedSearchCV.html}}, and hyperparameter tune the parameters \texttt{max\_depth}, \texttt{max\_features}, and \texttt{n\_estimators}. Once we discover the optimal hyperparameters, we retrain the model using the chosen parameters (on the same bootstrap sample) and evaluate it on the test set by adjusted $R^2$ measure. While prior studies typically measure the explanatory power of a constructed model by measuring its $R^2$ score on the training set, we do not do so as Any Liaw, maintainer of the \texttt{randomForest} R package explains, because of how a random forest model is constructed the $R^2$ of a random forest model calculated on a training set is always very close to 1 (typically in the 0.95 to 1.0 range). In addition, we use \textit{adjusted} version of the $R^2$ measure, which mitigates the bias introduced by the high number of features used in our model~\citep{Harrell15}. Since we generate 100 bootstrap samples, we obtain 100 adjusted $R^2$ values. We report summary statistics for this distribution of $R^2$ values.

%To evaluate the explanatory power of a model it is typical for researchers to calculate the goodness-of-fit of the model on the training data\gopi{ Add shane's papers}. However, since we use a random forest model, we do not Differently from linear regression models, the $R^2$ of a random forest model should not be calculated on a training set\footnote{An explanation by Andy Liaw, maintainer of the \texttt{randomForest} R package, is given at \url{https://stat.ethz.ch/pipermail/r-help/2010-October/257208.html}} (i.e., it should not be calculated on the same data that was used to train the model). By construction, the $R^2$ of a random forest model calculated on a training set is always very close to 1 (typically in the 0.95 to 1.0 range). 

%Due to the temporal aspect of our dataset, we also cannot calculate $R^2$ using random forest's out-of-bag (OOB) data nor other common model validation approaches, such as cross-validation and out-of-bag bootstrapping. If we used any of these options, we would be incurring into cases where a model is trained using a transaction $t_1$ that was processed at $timestamp(t_1)=x_1$ and tested on another transaction $t_2$ that was processed at $timestamp(t_2)=x_2$ and $x_1 > x_2$. That is, we would be training models with ``future'' data (data leakage problem) \goliva{Gopi might know a proper reference for this}.




\begin{figure}[!htbp]
\centering
    \includegraphics[width=0.8\linewidth]{prelim-study/model_validation_approach.pdf}
    \caption{Our model validation approach. RF stands for Random Forest and HP stands for hyperparameter.}
    \label{fig:model-validation}
\end{figure}

\smallskip \noindent \textbf{Results.} 
% \observation{Our random forest model achieves mean and median adjusted R\textsuperscript{2} scores of 0.48 and 0.50 respectively.} 
Our random forest model achieves mean and median adjusted R\textsuperscript{2} scores of 0.48 and 0.50 respectively. These scores indicate that our features explain approximately 50\% of the variance in processing times of the test data. We find these scores confirm the robust explanatory power of our features, demonstrating the stability of our models (\cite{Bird2011}, \cite{Jiarpakdee2021}, \cite{Mcintosh16}).  

In particular, they are compatible (and even sometimes outperform) adjusted $R^2$ scores reported in software engineering studies that built regression models with the purpose of understanding a certain phenomenon (\cite{Mcintosh16}, \cite{Jiarpakdee2021}, \cite{Bird2011}). For instance, \citet{Mcintosh16} built sophisticated regression models using restricted cubic splines to determine whether there is a relationship between (i) code review coverage and post-release defects, (ii) code review participation and post-release defects, and (iii) reviewer expertise and post-release defects. In total, the authors built 10 models and obtained adjusted $R^2$ scores that ranged from 0.20 to 0.67 (mean = 0.46, median = 0.41, sd = 0.17). In comparison, the median adjusted $R^2$ score of our model is 0.50, which sits higher than the median score achieved by their models. Most importantly, our score was computed on a \textit{held-out test set}, while theirs were computed on the \textit{train set}.

\goliva{**IMPORTANT** We should ideally do a residual analysis (check for randomness) or something to come up with an even stronger argument.}\gopi{Do we want to present a residual plot? or simply show MAE/AE?}\mike{To do, should we decide on which one we  will do?}

\mike{Removed the summary/declaration of our R2 scores}

% \begin{scriptsize}
% \begin{mybox}{Summary}
%     \textbf{\PrelimStudy}
%     \tcblower
%     Yes, since our random forest models achieve mean and median adjusted $R^2$ scores of 0.47 and 0.48 respectively a held-out test set.
% \end{mybox}
% \end{scriptsize}

==> rq.tex <==
\section{\RQ}
\label{sec:rq}

% !What features are more strongly associated with transaction processing times in Ethereum.?

%\mike{discussing with Gopi. at the moment the plots are still log transformed. for hte purpose of our paper, Gopi and I think we should try and remove the log transform on plots, so we can interpret them in real values). though it sounds like its ok either way. mentioning it here so we all remember}

\noindent \textbf{Motivation.} The Ethereum blockchain contains a plethora of features that potentially influence transaction processing times (e.g., miners, transaction's gas parameters, network utilization). Discovering the influence degree of each dimension and feature on the processing times of transactions in Ethereum enables us to understand and more importantly both enable and empower the development of cost-effective, next-generation \dapps~\citep{Oliva21}.% is a key step towards the construction of an accurate and explainable machine learning model for the prediction of processing times in Ethereum. 


%We address our research question by determining the features that are more strongly associated with transaction processing times.
\smallskip \noindent \textbf{Approach.} We employ a top-down approach with three steps to generate explanations from our model that determines the degree to which the studied dimensions and features impact the processing times of the transaction in ethereum. First, we perform a chunk test (step-1) on each feature dimension using the previously constructed models to define the levels of explanatory power that each dimension holds. Next, we compute a feature importance ranking using SHapley Additive exPlanations (SHAP) values and the Scott-Knott algorithm (step-2). Finally, we compute Partial Dependence Plots (PDPs) to investigate how the most important features of our model are driving the processing time predictions (step-3). Below, we describe our explanation approach in more detail:

\begin{itemize}[itemsep=3pt, wide = 0pt, topsep=3pt, listparindent=\parindent]
    \item \textit{(Step-1) Analysis of Dimension Importance via Chunk Tests and Scott-Knott.} The rationale behind a chunk test is to remove a group of features (e.g., all historical features) from an original model and observe the extent to which it impacts an evaluation measure of interest (e.g., the \textit{adjusted $R^2$}). For instance, if historical features are important, removing them from the model should yield a significant drop in the \textit{adjusted $R^2$} compared to the original full model. 
    
    To perform our chunk test, we reuse the model validation approach shown in Figure~\ref{fig:model-validation}. This time however, we build three additional random forest models for each bootstrap sample, each of which is constructed with one of the studied dimensions omitted (e.g., a model \textit{without} historical features). We refer to them as \textit{partial models}. Similar to Section~\ref{sec:model-construction}, we hyperparamter tune these models on the validation set and the retrain the model on the training set with the optimal parameters. We then have these partial models predict on the testing set and record their adjusted $R^2$ scores. Finally, we subtract these scores from that of the original model containing all features. We refer to this measure as the \textit{difference in adjusted $R^2$}. Since we have 100 bootstrap samples, we obtain 100 \textit{difference in adjusted $R^2$} scores for each partial model. We compare the score distributions of each partial model using boxplots.
    
    \item \textit{Step-2) Analysis of Feature Importance via SHAP and Scott-Knott.} We compute the SHAP value of each feature for each instance (dataset row). As a result, the importance of each feature is represented by a distribution of SHAP values. Next, we rank these feature importance distributions using the Scott-Knott (SK) algorithm. In the following, we explain these procedures in more detail.

	    \begin{itemize}[itemsep=3pt, wide = 0pt, topsep=3pt, listparindent=\parindent]
            
            \item \textit{Step-2a) SHapley Additive exPlanations (SHAP) computation.} To compute SHAP values, we first train a single random forest model on the entire \textit{train set} (28 consecutive days) using the procedures outlined in Section~\ref{sec:model-construction}. Next, we use the \texttt{TreeExplainer} API from the \texttt{shap} python package to compute the SHAP value of each feature for each dataset instance. As a result, each feature will have an associated SHAP value distribution of size $N$, where $N$ is the total number of rows in our train dataset. Finally, we convert these SHAP value distributions into \textit{absolute} SHAP value distributions. The rationale of such a conversion is that a feature $f_1$ with a SHAP value of $x$ is as important as a feature $f_2$ with a SHAP value of $-x$.

            %SHAP has been a groundbreaking interpretation technique for machine learning. Although the technique was proposed somewhat recently in 2017 by \citet{Lundberg17}, the paper has already received more than 2.6k citations as of July 2021\footnote{\url{https://www.researchgate.net/publication/317062430_A_Unified_Approach_to_Interpreting_Model_Predictions}}. A rigorous explanation of SHAP can be found in the original papers~\citep{Lundberg17,Covert20}. A more digestible explanation can be found in the \textit{Interpretable Machine Learning} book by Christoph Molnar~\citep{molnar2019}.

            \item \textit{Step 2b) Feature ranks from SHAP values.} We use the Scott-Knott algorithm (SK)~\citep{Scott74} to rank the distributions of absolute SHAP values generated in step-2b. We use Menzies's implementation of the SK algorithm~\citep{TimSK}, which (i) replaces the original parametric statistical tests with non-parametric ones and (ii) takes effect size into consideration (Cliff's Delta). Menzies's changes make the SK algorithm suitable to be used in the context of large datasets, where (i) p-values are close to meaningless without an accompanying effect size measure and (ii) few or even no assumptions can be made in terms of the shape of the distributions.
                   
            In our study, the SK computation leads to a feature ranking where the feature ranked \textit{first} is the one with the highest SHAP values. This ranking reflects the features order of influence that the studied features have on the transaction processing times in Ethereum platform. In contrast, the SHAP value computed for each dataset row reflect how the features influence the transaction processing time for that given transaction. We also note that there can be a rank tie between two or more features, which indicates that their underlying SHAP distributions are indistinguishable in practice (negligible effect size).

        \end{itemize}

    \item \textit{Step-3) Analysis of the relationship between top-ranked features and processing times via Partial Dependence Plots (PDP).} Once we discover what the top-ranked features are (step-2), we investigate them more closely via Partial Dependence Plots (PDPs). A PDP shows the marginal effect that a given feature has on the predicted outcome of a machine learning model. In particular, a PDP can show whether the relationship between the dependent feature (\textit{processing time} in our case) and a feature is linear, monotonic or more complex~\citep{molnar2019}. We use the \texttt{shap} python package to produce PDPs. We produce PDPs for the features belonging to the top-3 ranks. To ease interpretation, we back-transform the features (i.e., undo the log transformation) prior to PDP plotting.

\end{itemize}

\smallskip \noindent \textbf{Findings.} Our random forest model achieves mean and median adjusted R\textsuperscript{2} scores of 0.48 and 0.50 respectively. These scores indicate that our features explain approximately 50\% of the variance in processing times of the test data. We find these scores confirm the robust explanatory power of our features, demonstrating the stability of our models (\cite{Bird2011}, \cite{Jiarpakdee2021}, \cite{Mcintosh16}).  

\smallskip \noindent  \observation{The historical feature dimension is by far the most important one.} The result of the \textit{dimensions chunk test} is illustrated in Figure~\ref{fig:chunktest}. As the figure indicates, the random forest models without features from the historical dimension consistently hold the largest differences in adjusted R\textsuperscript{2} scores from the original random forest model, achieving a median difference of 0.41. In comparison, the median difference in adjusted R\textsuperscript{2} is only 0.04 for behavioral features and 0.01 for contextual features.

\begin{figure}[!htbp]
\centering
    \includegraphics[width=\linewidth]{rq/v2/chunktest.pdf}
    \caption{The distribution of differences in R\textsuperscript{2} scores between each of the models with a feature dimension omitted, and the model with all feature dimensions.}    
    \label{fig:chunktest}
\end{figure}

%\observation{The behavioral and contextual feature dimensions hold very little explanatory power overall.} Following our first observation, we find the models without features from the behavioral dimension achieve a median difference of 0.030 (ranked second), while the models without contextual features achieve a median difference of 0.015 (ranked third). Finally, we note that in some instances the removal of behavioral or contextual dimensions results in an increase in performance reflected by a negative difference in adjusted R\textsuperscript{2} scores, which is a result of the hyperparameter-tuned original model overfitting to the training data.

\observation{Recent transactional information is key in determining the processing time of a transaction.} Figure~\ref{fig:feature_importance} depicts the distribution of absolute SHAP values of each feature. As the figure indicates, the top-3 most important features are: \texttt{med\_num\_below\_120\_perc} (rank 1), \texttt{std\_num\_below\_120} (rank 2), \texttt{num\_same\_1\_perc} (rank 3). All these four features  fall into the \textit{historical dimension}, which is aligned with the results that we obtained from our chunk test (Figure~\ref{fig:chunktest}). Most importantly, all these features are engineered around information regarding the transactions processed within the previous 120 blocks (i.e., \textit{recent} transaction informational).

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{rq/v2/shap_values_dist_ranking.pdf}
    \caption{The distribution of absolute SHAP values per feature. Features are grouped according to their importance rank. Due to the high skewness of the data, we apply a log(x+1) transformation to the y-axis.}    
    \label{fig:feature_importance}
\end{figure}

\observation{The important features can be subject to change depending on the feature values of the transaction at hand.} As depicted in Figure~\ref{fig:feature_importance}, we note some variation in the SHAP values generated for each feature across each instance of the dataset. For example, although the top feature \textit{med\_num\_below\_120\_perc} contains the highest median SHAP value, we observe the existence of instances in that distribution with low SHAP values. The opposite scenario is also true. We also observe that certain low-ranked features (e.g., \texttt{med\_pending\_pool\_120}) might contain very high SHAP values for certain instances (outliers).This result indicates that, depending on the exact feature values of a given transaction, certain globally top-ranked features can be considered irrelevant to that transaction and vice-versa. \gopi{Fig 10 and Fig 11 can be incorporated here?}\mike{Maybe, waht do you think @Gustvao?}\goliva{yep, agree (just Fig 11 is enough). see my comment for Implication 1}
%(global importance versus local importance).

% \mike{But how much do they vary? we can use kendal tau here again to measure variation here. wondering if we should apply windows here, like separate the data into windows, use SK to rank the dist. of SHAP values in each window. then use kendall tau compare them to the final ranks. otherwise we can rank shap values for each instance, and just use kendal tau from there. Or we can just use the PEPs/waterfall. can also think about more to write here}.

\observation{The PDP of the med\_num\_below\_120\_perc suggests that there is gas price  at which transactions are processed closest to the fastest speed possible (and thus increasing such a price will *not* further reduce the processing time.)} %In Figure~\ref{fig:pdp-1}, we show the PDP for \texttt{med\_num\_below\_120\_perc} (rank 1). By construction, when the value of this feature is close 0\% for a given transaction $t$, it means the gas price of $t$ is very small \textit{relative} to the prices of the transactions in at least half of the prior 120 blocks. Hence, the processing time of $t$ is expected to be high. As the value of \texttt{med\_num\_below\_120\_perc} increases, transactions are expected to be processed faster. 
The PDP depicted in Figure~\ref{fig:pdp-1} leads to several insights. First, the range of the y-axis indicates that changes in \texttt{med\_num\_below\_120\_perc} indeed have a large influence on the predicted processing times. Second, we notice a sharp decline in processing time as soon as feature values become greater than zero. That is, let $p(B)$ be the lowest gas price used by a transaction inside a mined block B. Let $p(t)$ be the gas price of a transaction $t$. Setting $p(t)$ such that $p(t) > p(B)$ is true for at least half of the 120 most recently mined blocks already provides a speed boost in transaction processing time. Third, the PDP indicates that the estimated processing time decreases as feature values increase (i.e., as the gas price of the current transaction becomes higher those from recent transactions), but only up until a certain point. At 64\%, a plateau is reached and processing times do not tend to decrease any further. 
%Upon close inspection, we note that at a feature value of 64\%, processing times are close to 0.58 minutes = 35 seconds. According to Etherscan, the daily average block time (i.e., the time between two consecutive mined blocks) is approximately 13 seconds for the 28 consecutive days included in our \textit{train set} window. In other words, for feature values higher than 64\% (and smaller than 95\%), the predicted processing time is already close to the minimum possible processing time observed in Ethereum during the train set window. 
Most importantly, this result is telling us that (i) increasing the gas price beyond a certain value $x$ does not tend to reduce processing times any further and (ii) the value of $x$ is dependent on the prices of the transaction in the prior 120 blocks (otherwise the \texttt{gas\_price\_gwei} would be more important than \texttt{med\_num\_below\_120\_perc}). Finally, we observe that feature values beyond 95\% seem to lead to an increase in the estimated processing times, which is counterintuitive. However, a closer look at the density plot (top of Figure~\ref{fig:pdp-1}) reveals that a feature value of 95\% corresponds to the 90th percentile of the distribution. As feature values approach the right tail of the distribution, the model predictions tend to become fuzzier due to the lack of enough training data. Hence, we attribute the increase in processing time to the limited availability of corresponding training data.

%Our model seems to be penalizing transactions with very high gas prices. A transaction $t$ with a very high gas price signals a desire for urgency in the processing of such a transaction. We conjecture that in an urgency scenario, the same transaction issuer might be issuing multiple transactions simultaneously, which increases the chances that one transaction will get blocked due to another pending transaction with a lower \textit{nonce} (see \texttt{tx\_nonce} in Table~\ref{tab:features}).

\begin{figure}[!htbp]
\centering
    \includegraphics[width=\linewidth]{rq/med_num_below_120_perc.pdf}
    \caption{A partial dependence plot for the \textit{med\_num\_below\_120\_perc} feature and transaction processing time.}    
    \label{fig:pdp-1}
\end{figure}

\observation{The predicted processing time decreases as the values of std\_num\_below\_120 increase (except for very large values of the latter).} In Figure~\ref{fig:pdp-2}, we see the relationship between \texttt{std\_num\_below\_120} (standard deviation of the percentage of transactions processed per block, in the previous 120 blocks, with a gas price below the current transaction) and the estimated processing time. First, the range of the y-axis indicates that changes in the feature values are associated with large changes in the estimated processing time. Next, we observe that the relationship between the feature of interest and the estimated processing time takes the form of a U-shaped curve. Generally speaking, up until 28\%, the more variation there is in the percentage of recently processed transactions with gas price lower that the current transaction, the higher the bias towards the prediction of a shorter processing time. However, from 28\% onwards, the estimated processing time sharply increases. Similarly to Figure~\ref{fig:pdp-1}, such an increase is associated with the remaining 10\% of the data (note the density plot). Hence, we once again attribute the aforementioned increase to the limited availability of corresponding training data.
%the model understands that there is too much variation in the data and starts biasing the predictions in the opposite direction (but much quicker). 

\begin{figure}[!htbp]
\centering
    \includegraphics[width=\linewidth]{rq/std_num_below_120_perc.pdf}
    \caption{A partial dependence plot for the \textit{std\_num\_below\_120} feature and transaction processing time.\mike{I need to fix the name of the feature in this figure, as well as its name in teh waterfall plots if we continue using them}}    
    \label{fig:pdp-2}
\end{figure}

\observation{The predicted processing time decreases as the values of num\_same\_1\_perc increase (except for very large values of the latter).} Figure~\ref{fig:pdp-3} displays the relationship between \texttt{num\_same\_1\_perc} and the predicted processing times. The feature in question refers to the percentage of transactions in the prior block that were assigned the same gas price as the current transaction. Since feature values are extremely right-skewed, we apply a log(X+1) transformation to the x-axis. First, we note that the range in the y-axis is much smaller compared to the two previously shown PDPs. Such a result corroborates the feature ranking depicted in Figure~\ref{fig:feature_importance}, which indicates that the absolute SHAP values of \texttt{num\_same\_1\_perc} are significantly smaller than those from \texttt{med\_num\_below\_120\_perc}. Therefore, we conclude that features with rank 3 and higher have much lower influence on the predicted outcome by themselves. Having said that, we observe that the predicted processing times do decrease as feature values increase (up to the 90th percentile again). Such a behavior makes sense: as the percentage of transactions in the previous block with the same gas price as the current transaction increases, so should the processing time (as these transactions should be of similar priority to miners). From the 90th percentile onward, we observe the same fuzzier, upward trend in predicted processing times.

\begin{figure}[!htbp]
\centering
    \includegraphics[width=\linewidth]{rq/num_same_1_perc.pdf}
    \caption{A partial dependence plot for the \textit{num\_same\_1\_perc} feature and transaction processing time.}
    \label{fig:pdp-3}
\end{figure}

\begin{scriptsize}
\begin{mybox}{Summary}
  \textbf{\RQ}
  \tcblower
  The features that consistently best characterize transaction processing times include features from the historical dimension. In particular:
  \begin{itemize}[topsep = 3pt, itemsep = 3pt, label=\textbullet, wide = 0pt]
    
    \item The historical feature dimension consistently holds the highest level of explanatory power overall among the three studied dimensions. The behavioral and contextual feature dimensions hold very little explanatory power overall.
    
    \item The \textit{med\_num\_below\_120\_perc}, \textit{std\_num\_below\_120}, and \textit{num\_same\_1\_perc} features consistently hold the strongest explanatory power. The relationship between each of these features and the estimated processing time generally assumes the form of a monotonic decreasing function.
    \item The relationship between \textit{med\_num\_below\_120\_perc} and the estimated processing time suggests transactions in the prior 120 blocks are most important in estimating processing time, and that transactions with increasing gas prices result in diminishing returns in processing times. \mike{Observation to be reviewed.}
    \item The globally important features (i.e., across the entire dataset) might differ from the locally important features (i.e., those associated with a single dataset instance).
    
  \end{itemize}
\end{mybox}
\end{scriptsize}

% Ideas/notes
% 1. PEPs/Nomogram would be really good so we can say when x feature increeases, the resulting predicting inc/dec. Especially good for the 2nd feature which measures the standard deviation, and also tx nonce
% 2. We can use kendall tau like we did before to find windows that deviate from the ranks resulting from SK. We can't really use SK to rank a single instance (i think), so maybe we need another ranking approach for that. 
% If we do this, then can the waterfall plots resulting from the "representative" and "deviate" windows tell use what a PEP/Nomogram would? (eg x inc, y dec) 
% Is this just plotting value of feature vs predicted value?

% 3. Rank the R2 difference distributions for the chunk test (SK)
% Might want a plot similar to the feature importance one
% Do we want plots for the R2 scores of those chunked models as well? Maybe just a table

% All of these features are from historical dimension
% All of these features are engineered using gas price data, but not gas limit data
% The percentage of txs in the previous block with the same gas price as the tx in question, and the processing time the most recent tx within the previous 120 blocks which contains a gas price closest to the tx in question are tied for rank 3
% Three of the four features include data regarding the # of identical txs processed in the recent past

% Gas price feature is rank 5, though gas limit is ranked 21
% The std of gas usage consumed within the previous 120 blocks by the same target contract function as the tx in question is also ranked 24

% The highest rank of a feature related to Blockchain difficulty is ranked 15
% The highest rank of a feature related to pending pool is rank 15

% Tx nonce is ranked 6? do miners prioritize/expect experience over gas limit? can we check if these two metrics  corr? 0.2656482355 nonce vs tx limit
% 0.127650906 nonce vs gas price 
% 0.0447394458 gas price and gas limit

==> templates/my-emse-template/abstract.tex <==
\begin{abstract}

\keywords{Smart Contracts, Ethereum, Blockchain}
\end{abstract}


==> templates/my-emse-template/background.tex <==
\section{Background}
\label{sec:backgroud}

==> templates/my-emse-template/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
  
\noindent [Relevance of topic addressed in the paper]

\medskip \noindent [What was done in one sentence, including the topic of each RQ and the data used]

\medskip \noindent We conclude that [conclusions that derive from results, focusing on implications to the customer of the paper]

==> templates/my-emse-template/data-collection.tex <==
\section{Data Collection}
\label{sec:data-collection}


\begin{mybox}{Summary}
	\begin{itemize}[itemsep = 3pt, label=\textbullet]
		\item Data collection starting day: 15-09-2018 (dd-mm-yyyy)
		\item Data sources: 
		\item Pieces of data collected: 
	\end{itemize}
\end{mybox}

==> templates/my-emse-template/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> templates/my-emse-template/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\noindent [Context]

\medskip \noindent [Motivation/Problem.]

\medskip \noindent [What we did.]

\medskip \noindent (RQs.) In the following, we list our research questions and key observations:

\medskip

\noindent \textbf{RQ1) \RQOne} [Summarized approach] We observed that:

\smallskip \noindent \textit{Key results}

\medskip

\noindent \textbf{RQ2) \RQTwo}  [Summarized approach] We observed that:

\smallskip \noindent \textit{Key results}

\medskip

\noindent \textbf{RQ3) \RQThree}  [Summarized approach] We observed that:

\smallskip \noindent \textit{Key results}

\medskip

In summary, our empirical results led us to conclude that: \textit{The one thing reader should never forget after reading the paper.}

\subsection{Paper Organization}

The remainder of this paper is organized as follows. Section \ref{sec:backgroud} [bla]. Section \ref{sec:data-collection} explains the data collection procedures that we employed to [bla]. Section \ref{sec:results} presents and discusses the results of our research questions. Section \ref{sec:related-work} presents the different perspectives from which prior research has [bla]. Section \ref{sec:threats-to-validity} discusses the threats to the validity of our study. Finally, Section \ref{sec:conclusion} concludes the paper by summarizing our observations.

==> templates/my-emse-template/related-work.tex <==
\section{Related Work}
\label{sec:related-work}


==> templates/my-emse-template/results-rq1.tex <==
\subsection{RQ1: \RQOne}
\label{subsec:rq1}

\noindent \textbf{Motivation.} 

\medskip \noindent \textbf{Approach.} 

\medskip \begin{observation}{Bold statement}\label{obs:1}
	Here is the result
\end{observation}

\medskip \begin{observation}{Bold statement}\label{obs:2}
	Here is the result
\end{observation}

\medskip \begin{observation}{Bold statement}\label{obs:3}
	Here is the result
\end{observation}

\begin{mybox}{RQ1: \RQOne}
	One sentence summary. In particular:
	
	\begin{itemize}[itemsep = 3pt, label=\textbullet]
		\item Observation \ref{obs:1}
		\item Observation \ref{obs:2}
		\item Observation \ref{obs:3}
	\end{itemize}
	
\end{mybox}



==> templates/my-emse-template/results-rq2.tex <==
\subsection{RQ2: \RQTwo} 
\label{subsec:rq2}

\noindent \textbf{Motivation.} 

\medskip \noindent \textbf{Approach.} 

\medskip \begin{observation}{Bold statement}\label{obs:4}
	Here is the result
\end{observation}

\medskip \begin{observation}{Bold statement}\label{obs:5}
	Here is the result
\end{observation}

\medskip \begin{observation}{Bold statement}\label{obs:6}
	Here is the result
\end{observation}

\begin{mybox}{RQ2: \RQTwo}
	One sentence summary. In particular:
	
	\begin{itemize}[itemsep = 3pt, label=\textbullet]
		\item Observation \ref{obs:4}
		\item Observation \ref{obs:5}
		\item Observation \ref{obs:6}
	\end{itemize}
	
\end{mybox}

==> templates/my-emse-template/results-rq3.tex <==
\subsection{RQ3: \RQThree}
\label{subsec:rq3}


\noindent \textbf{Motivation.} 

\medskip \noindent \textbf{Approach.} 

\medskip \begin{observation}{Bold statement}\label{obs:7}
	Here is the result
\end{observation}

\medskip \begin{observation}{Bold statement}\label{obs:8}
	Here is the result
\end{observation}

\medskip \begin{observation}{Bold statement}\label{obs:9}
	Here is the result
\end{observation}

\begin{mybox}{RQ3: \RQThree}
	One sentence summary. In particular:
	
	\begin{itemize}[itemsep = 3pt, label=\textbullet]
		\item Observation \ref{obs:7}
		\item Observation \ref{obs:8}
		\item Observation \ref{obs:9}
	\end{itemize}
	
\end{mybox}


==> templates/my-emse-template/results.tex <==
\section{Exploratory Study}
\label{sec:results}

\input{results-rq1}
\input{results-rq2}
\input{results-rq3}

==> templates/my-emse-template/solidity-highlighting.tex <==
% Copyright 2017 Sergei Tikhomirov, MIT License
% https://github.com/s-tikhomirov/solidity-latex-highlighting/

\usepackage{listings, xcolor}

\definecolor{customcolor}{rgb}{1,1,1}

\lstdefinelanguage{Solidity}{
	keywords=[1]{anonymous, assembly, assert, balance, break, call, callcode, case, catch, class, constant, continue, contract, debugger, default, delegatecall, delete, do, else, emit, event, export, external, false, finally, for, function, gas, if, implements, import, in, indexed, instanceof, interface, internal, is, length, library, log0, log1, log2, log3, log4, memory, modifier, new, payable, pragma, private, protected, public, pure, push, require, return, returns, revert, selfdestruct, send, storage, struct, suicide, super, switch, then, this, throw, transfer, true, try, typeof, using, value, view, while, with, addmod, ecrecover, keccak256, mulmod, ripemd160, sha256, sha3}, % generic keywords including crypto operations
	keywordstyle=[1]\color{blue}\bfseries,
	keywords=[2]{address, bool, byte, bytes, bytes1, bytes2, bytes3, bytes4, bytes5, bytes6, bytes7, bytes8, bytes9, bytes10, bytes11, bytes12, bytes13, bytes14, bytes15, bytes16, bytes17, bytes18, bytes19, bytes20, bytes21, bytes22, bytes23, bytes24, bytes25, bytes26, bytes27, bytes28, bytes29, bytes30, bytes31, bytes32, enum, int, int8, int16, int24, int32, int40, int48, int56, int64, int72, int80, int88, int96, int104, int112, int120, int128, int136, int144, int152, int160, int168, int176, int184, int192, int200, int208, int216, int224, int232, int240, int248, int256, mapping, string, uint, uint8, uint16, uint24, uint32, uint40, uint48, uint56, uint64, uint72, uint80, uint88, uint96, uint104, uint112, uint120, uint128, uint136, uint144, uint152, uint160, uint168, uint176, uint184, uint192, uint200, uint208, uint216, uint224, uint232, uint240, uint248, uint256, var, void, ether, finney, szabo, wei, days, hours, minutes, seconds, weeks, years},	% types; money and time units
	keywordstyle=[2]\color{teal}\bfseries,
	keywords=[3]{block, blockhash, coinbase, difficulty, gaslimit, number, timestamp, msg, data, gas, sender, sig, value, now, tx, gasprice, origin},	% environment variables
	keywordstyle=[3]\color{violet}\bfseries,
	identifierstyle=\color{black},
	sensitive=false,
	comment=[l]{//},
	morecomment=[s]{/*}{*/},
	commentstyle=\color{gray}\ttfamily,
	stringstyle=\color{red}\ttfamily,
	morestring=[b]',
	morestring=[b]"
}

\lstset{
	language=Solidity,
	backgroundcolor=\color{customcolor},
	extendedchars=true,
	basicstyle=\footnotesize\ttfamily,
	showstringspaces=false,
	showspaces=false,
	numbers=left,
	numberstyle=\footnotesize,
	numbersep=9pt,
	tabsize=2,
	breaklines=true,
	showtabs=false,
	captionpos=b,
	xleftmargin=2em,
	frame=single,
	framexleftmargin=2em
}

==> templates/my-emse-template/threats.tex <==
\section{Threats to Validity}
\label{sec:threats-to-validity}

\noindent \textbf{Construct Validity.} 

\medskip \noindent \textbf{Internal Validity.} 

\medskip  \noindent \textbf{External Validity.}
